Notes on Probability Theory

This is the first of the proposed sets of notes to be published in the website Gonit Sora (http://gonitsora.com). The notes will hopefully be able to help the students to learn their subject in an easy and comprehensible way. These notes are aimed at mimicking exactly what would be typically taught in a one-semester course at a college or university. The level of the notes would be roughly at the undergraduate level. The present sets of notes are not yet complete and this is the second version that is being posted. These notes contain very few proofs and only state the important results in Probability Theory. These notes are based on the course taught at Tezpur University, Assam, India by Dr. Santanu Dutta. There may be some errors and typos in these notes which we hope the reader would bring to our notice.

==> nomenclature.tex <==
\setlongtables
\renewcommand{\arraystretch}{1.5}
\begin{longtable}{l l}
\caption*{\textbf{NOMENCLATURE}}\\
%\hline
SPP   &       Singular Perturbation Problem\\
SPDDE  &      Singularly Perturbed Differential-Difference Equation\\
BVP   &       Boundary-Value Problem\\
FMM   &       Fitted Mesh Method\\
ODE   &       Ordinary Differential Equation\\
PDE   &       Partial Differential Equation\\

\end{longtable}


==> titlepage.tex <==
\thispagestyle{empty}
\begin{center}
\baselineskip=24pt {{\sf\Huge Spectra of Weighted Directed Graphs}}

                      \vspace*{3cm}
                   { \large\sf A thesis submitted} \\

                     { \sf \large    in Partial Fulfillment of the
                         Requirements}\\

                         { \sf \large  for the Degree of}\\
                        %\vspace{5mm}
                   {\Large \sf Doctor of Philosophy} \\
                      \vspace{18mm}
                   {\em  \Large {by}} \\ \vspace{3mm}
             {\Huge \texttt{Debajit Kalita}} \\
           %   {\bf Roll Number: 06612303}\\
                   \vspace{1.2cm}


{\epsfig{file=iitg_logo.eps, width=3.5cm,height=3.5cm,angle=0}}


                   \vspace*{1cm}
\baselineskip=24pt
    {\em      \large   to the} \\
                 {\Large \sf {Department of Mathematics}} \\
{\Large      \sf {Indian Institute of Technology Guwahati}}\\
{\Large  \sf    Guwahati-781039, India}\\
{\large                        \sf{August, 2011}}
\end{center}
%\clearpage

